Unveiling the Political Agenda of the European Parliament Plenary: A Topical Analysis

This study analyzes political interactions in the European Parliament (EP) by considering how the political agenda of the plenary sessions has evolved over time and the manner in which Members of the European Parliament (MEPs) have reacted to external and internal stimuli when making Parliamentary speeches. It does so by considering the context in which speeches are made, and the content of those speeches. To detect latent themes in legislative speeches over time, speech content is analyzed using a new dynamic topic modeling method, based on two layers of matrix factorization. This method is applied to a new corpus of all English language legislative speeches in the EP plenary from the period 1999-2014. Our findings suggest that the political agenda of the EP has evolved significantly over time, is impacted upon by the committee structure of the Parliament, and reacts to exogenous events such as EU Treaty referenda and the emergence of the Euro-crisis have a significant impact on what is being discussed in Parliament.

==> regtab.tex <==
\begin{table}[!b]
	\centering
	\scriptsize{
\def\sym#1{\ifmmode^{#1}\else\(^{#1}\)\fi}
\begin{tabular}{l*{1}{cc}}
\hline	%\hline
 %                   &\multicolumn{2}{c}{}           \\
                    &\multicolumn{2}{c}{Model 1}          \\
\hline
Speech count component       &                     &            \\
Party L-R           &       1.002         &      (0.14)\\
MEP defector to nat. party &       0.626         &     (-1.39)\\
MEP defector to EP group &       0.704         &     (-0.93)\\
EP leadership     &       0.941         &     (-1.47)\\
Chair of topic-relevant committee &       1.173\sym{*}  &      (2.40)\\
Rapporteur of topic-relevant committee &       1.582\sym{***}&      (9.76)\\
Member of topic-relevant committee &       2.077\sym{***}&     (18.10)\\
MEP's total speeches &       1.002\sym{***}&     (30.86)\\
Percent Speeches translated &       1.003\sym{**} &      (3.27)\\
Constant            &       8.785\sym{***}&     (14.23)\\
\hline
Zero-inflated component             &                     &            \\
Party L-R           &       1.039\sym{*}  &      (2.38)\\
MEP defector to nat. party &       0.248\sym{*}  &     (-2.44)\\
MEP defector to EP group&       4.820\sym{*}  &      (2.03)\\
EP leadership     &       1.234         &      (1.15)\\
Chair of topic-relevant comm &       0.721         &     (-1.08)\\
Rapporteur of topic-relevant comm &       0.255\sym{***}&     (-8.66)\\
Member of topic-relevant comm &       0.259\sym{***}&    (-12.37)\\
MEP's total speeches &       0.976\sym{***}&    (-15.83)\\
Percent Speeches in English &       0.996\sym{**} &     (-2.75)\\
Constant            &       0.416\sym{***}&     (-3.33)\\
\hline
%lnalpha             &                     &            \\
Constant            &       1.090\sym{**} &      (3.29)\\
\hline
%Country, EP group and  &                     &            \\
%Topic fixed effects excluded &                     &            \\
%\hline
Observations        &       34485         &            \\
\hline\hline
\multicolumn{3}{l}{Exponentiated coefficients; \textit{t} statistics in parentheses}\\
\multicolumn{3}{l}{\sym{*} \(p<0.05\), \sym{**} \(p<0.01\), \sym{***} \(p<0.001\)}\\
\end{tabular}
}
\caption{Zero-inflated negative binomial regression model for count of MEP speeches on a given topic. Country, EP group and topic fixed effects excluded from table.}
\label{tab:regtab}
\end{table}


==> tables_extra.tex <==
\newpage
\begin{table*}[h]
\centering
\scriptsize{
\begin{tabular}{|l|l|l|r|r|}
\hline
\textbf{\#} & \textbf{Short Label}                       & \textbf{Top 10 Terms}                                                                                & \textbf{Freq.} & \textbf{Per.} \\\hline
1              & Plenary administration               & president, european, political, resumption, resolution, continuation, business, adoption, union, ppe          & 57             & 11.27\%       \\
2              & Human rights                         & rights, human, fundamental, freedom, democracy, law, charter, resolution, union, violation                    & 52             & 8.53\%        \\
3              & Financial crisis                     & financial, crisis, economic, market, european, supervision, bank, perspective, fund, banking                  & 13             & 1.62\%        \\
4              & Gender equality                      & woman, equality, gender, equal, violence, discrimination, against, work, opportunity, life                    & 50             & 3.70\%        \\
5              & Commission questions                 & commission, commissioner, work, legislative, reform, subject, programme, case, annex, censure                 & 30             & 3.66\%        \\
6              & Energy                               & energy, gas, renewable, efficiency, supply, source, electricity, market, target, project                      & 36             & 3.18\%        \\
7              & Consumer protection                  & consumer, market, protection, internal, labelling, credit, regulation, single, product, network               & 36             & 3.71\%        \\
8              & Fisheries                            & fishery, fishing, fish, stock, fisherman, fleet, sea, common, policy, measure                                 & 34             & 2.27\%        \\
9              & Council Presidency                   & council, presidency, minister, brussels, european, regulation, common, cod, subject, summit                   & 24             & 2.47\%        \\
10             & Liberalising services                & service, market, public, postal, competition, internal, interest, liberalisation, sector, general             & 23             & 1.96\%        \\
11             & Trade 1 - Trade partnerships         & agreement, partnership, morocco, trade, negotiation, data, cooperation, association, korea, fishery           & 18             & 2.58\%        \\
12             & Budget                               & budget, draft, financial, eur, general, budgetary, section, committee, money, fund                            & 28             & 3.06\%        \\
13             & Transport                            & transport, railway, rail, passenger, road, network, freight, system, train, infrastructure                    & 19             & 1.38\%        \\
14             & Future of Europe                     & europe, union, european, states, citizen, enlargement, government, constitution, candidate, policy            & 22             & 2.77\%        \\
15             & Turkish accession                    & turkey, turkish, accession, progress, cyprus, negotiation, union, membership, croatia, macedonia              & 20             & 1.61\%        \\
16             & Research                             & research, programme, innovation, framework, funding, industry, technology, development, cell, institute       & 15             & 1.01\%        \\
17             & CFSP                                 & security, policy, defence, common, foreign, military, nato, immigration, aspect, european                     & 19             & 1.76\%        \\
18             & Russia                               & russia, russian, relation, summit, georgia, union, chechnya, partnership, eastern, cooperation                & 15             & 1.52\%        \\
19             & Social policy                        & social, employment, economic, worker, policy, labour, growth, economy, pension, jobs                          & 34             & 4.18\%        \\
20             & Israel/Palestine                     & palestinian, east, peace, middle, israeli, aid, palestine, international, state, government                   & 17             & 1.21\%        \\
21             & Healthcare                           & health, patient, environment, safety, public, care, healthcare, action, disease, mental                       & 18             & 0.99\%        \\
22             & Agriculture                          & agricultural, farmer, rural, agriculture, cap, milk, production, market, development, common                  & 27             & 1.94\%        \\
23             & Animal health and welfare            & animal, welfare, protection, meat, scientific, feed, ban, transport, control, plant                           & 14             & 0.96\%        \\
24             & Climate change                       & climate, emission, change, greenhouse, gas, trading, aviation, target, copenhagen, global                     & 14             & 1.47\%        \\
25             & Justice and home affairs             & committee, affairs, legal, petition, regulation, internal, ombudsman, market, citizen, statute                & 19             & 1.45\%        \\
26             & Child protection                     & child, internet, pornography, sexual, school, exploitation, young, victim, education, crime                   & 14             & 0.94\%        \\
27             & Promoting democracy                  & political, party, european, statute, financing, democracy, funding, election, democratic, government          & 11             & 0.91\%        \\
28             & Nuclear proliferation                & nuclear, iran, power, plant, safety, weapon, resolution, station, proliferation, decommissioning              & 10             & 0.56\%        \\
29             & Adjusting to globalisation           & fund, globalisation, egf, worker, adjustment, mobilisation, european, redundant, application, eur             & 15             & 1.62\%        \\
30             & Food safety                          & food, consumer, safety, farmer, additive, agricultural, aid, chain, flavouring, production                    & 14             & 1.51\%        \\
31             & Council Presidency program           & presidency, programme, minister, irish, prime, finnish, presentation, british, italian, swedish               & 9              & 0.49\%        \\
32             & Trade 2 - WTO and aid                & trade, wto, world, development, developing, international, negotiation, aid, free, relation                   & 19             & 2.12\%        \\
33             & Air transport                        & air, passenger, transport, aviation, airport, traffic, airline, flight, sky, single                           & 10             & 0.54\%        \\
34             & Drugs                                & drug, sport, centre, addiction, monitoring, precursor, convention, croatia, emcdda, young                     & 9              & 0.27\%        \\
35             & Tax                                  & tax, vat, taxation, rate, system, fraud, states, evasion, car, transaction                                    & 11             & 1.38\%        \\
36             & Waste management                     & waste, recycling, directive, packaging, management, environment, electronic, fuel, environmental, radioactive & 13             & 0.62\%        \\
37             & Enlargement                          & romania, accession, bulgaria, enlargement, progress, croatia, union, corruption, reform, romanian             & 7              & 0.49\%        \\
38             & Euro crisis                          & euro, economic, growth, stability, pact, bank, policy, monetary, economy, ecb                                 & 17             & 2.45\%        \\
39             & Education \& Culture                 & programme, education, culture, language, cultural, youth, sport, learning, young, training                    & 21             & 1.78\%        \\
40             & European agencies                    & agency, european, safety, rating, control, reconstruction, regulation, implementation, credit, maritime       & 5              & 0.57\%        \\
41             & Water                                & water, bathing, quality, resource, public, directive, management, mediterranean, groundwater, drinking        & 7              & 0.33\%        \\
42             & The Balkans                          & kosovo, serbia, balkan, resolution, bosnia, albania, iceland, herzegovina, macedonia, process                 & 12             & 0.38\%        \\
43             & Foreign elections                    & ukraine, election, belarus, resolution, democratic, ukrainian, democracy, quaestor, union, presidential       & 10             & 0.46\%        \\
44             & Terrorism                            & terrorism, against, terrorist, iraq, fight, united, international, war, combating, states                     & 9              & 0.83\%        \\
45             & Maritime issues                      & port, sea, maritime, safety, ship, accident, oil, vessel, transport, inspection                               & 10             & 0.54\%        \\
46             & Criminal matters  & data, protection, crime, citizen, criminal, law, states, personal, justice, organised                         & 15             & 1.04\%        \\
47             & Product labelling/regulation     & product, medicinal, medicine, tobacco, labelling, safety, consumer, regulation, organic, advertising          & 11             & 0.91\%        \\
48             & Roma                                 & roma, strategy, discrimination, minority, resolution, education, european, integration, freedom, school       & 5              & 0.38\%        \\
49             & Regional funds                       & policy, region, cohesion, development, regional, strategy, structural, fund, economic, area                   & 22             & 2.41\%        \\
50             & Trade with China                     & china, textile, chinese, industry, relation, sector, clothing, arm, import, tourism                           & 6              & 0.26\%        \\
51             & Natural disasters                    & forest, fire, disaster, natural, solidarity, aid, flood, prevention, affected, greece                         & 9              & 0.52\%        \\
52             & Foot and mouth                       & disease, mouth, foot, vaccination, outbreak, crisis, animal, commissioner, bse, measure                       & 7              & 0.33\%        \\
53             & Court issues                         & court, auditor, justice, annual, institution, criminal, ombudsman, international, judge, states               & 6              & 0.41\%        \\
54             & Schengen and borders                 & border, schengen, system, states, asylum, si, area, acquis, application, immigration                          & 12             & 1.57\%        \\
55             & EU directives                        & directive, worker, legislation, company, work, environmental, working, states, law, market                    & 13             & 1.42\%        \\
56             & Road safety                          & road, safety, vehicle, transport, system, driver, accident, motor, noise, ecall                               & 12             & 0.79\%        \\
57             & Treaties and referenda               & treaty, constitution, lisbon, citizen, referendum, constitutional, european, irish, convention, national      & 12             & 0.89\% 
\\\hline      
\end{tabular}
}
\caption{Full list of 57 dynamic topics discovered in the European Parliament English speeches corpus. For each dynamic topic, we report a manually-assigned short label, the top 10 terms, the frequency of the topic (\ie number of time windows in which it appeared), and the percentage of speeches from the complete corpus associated with the topic.}
\label{tab:topics}
\end{table*}

\newpage
\begin{table*}[h]
\centering
\scriptsize{
\begin{tabular}{|l|l|l|c|c|}
\hline
\textbf{Topic} & \textbf{Short Label}             & \textbf{Top 10 Terms}                                                                          & \textbf{Coh.} & \textbf{Freq.} \\\hline
13             & Transport                        & transport, railway, rail, passenger, road, network, freight, system, train, infrastructure              & 0.54          & 19             \\
42             & The Balkans                      & kosovo, serbia, balkan, resolution, bosnia, albania, iceland, herzegovina, macedonia, process           & 0.50          & 12             \\
33             & Air transport                    & air, passenger, transport, aviation, airport, traffic, airline, flight, sky, single                     & 0.48          & 10             \\
29             & Adjusting to globalisation       & fund, globalisation, egf, worker, adjustment, mobilisation, european, redundant, application, eur       & 0.47          & 15             \\
6              & Energy                           & energy, gas, renewable, efficiency, supply, source, electricity, market, target, project                & 0.47          & 36             \\
39             & Education and culture             & programme, education, culture, language, cultural, youth, sport, learning, young, training              & 0.43          & 21             \\
8              & Fisheries                        & fishery, fishing, fish, stock, fisherman, fleet, sea, common, policy, measure                           & 0.43          & 34             \\
2              & Human rights                     & rights, human, fundamental, freedom, democracy, law, charter, resolution, union, violation              & 0.43          & 52             \\
45             & Maritime issues                  & port, sea, maritime, safety, ship, accident, oil, vessel, transport, inspection                         & 0.43          & 10             \\
21             & Healthcare                       & health, patient, environment, safety, public, care, healthcare, action, disease, mental                 & 0.42          & 18             \\
26             & Child protection                 & child, internet, pornography, sexual, school, exploitation, young, victim, education, crime             & 0.42          & 14             \\
56             & Road safety                      & road, safety, vehicle, transport, system, driver, accident, motor, noise, ecall                         & 0.41          & 12             \\
16             & Research                         & research, programme, innovation, framework, funding, industry, technology, development, cell, institute & 0.41          & 15             \\
15             & Turkish accession                & turkey, turkish, accession, progress, cyprus, negotiation, union, membership, croatia, macedonia        & 0.41          & 20             \\
35             & Tax                              & tax, vat, taxation, rate, system, fraud, states, evasion, car, transaction                              & 0.41          & 11             \\
32             & Trade - WTO and aid            & trade, wto, world, development, developing, international, negotiation, aid, free, relation             & 0.39          & 19             \\
47             & Product labelling and regulation & product, medicinal, medicine, tobacco, labelling, safety, consumer, regulation, organic, advertising    & 0.39          & 11             \\
11             & Trade - Trade partnerships     & agreement, partnership, morocco, trade, negotiation, data, cooperation, association, korea, fishery     & 0.39          & 18             \\
49             & Regional funds                   & policy, region, cohesion, development, regional, strategy, structural, fund, economic, area             & 0.39          & 22             \\
17             & CFSP                             & security, policy, defence, common, foreign, military, nato, immigration, aspect, european               & 0.39          & 19            \\\hline
\end{tabular}
}
\caption{List of top 20 dynamic topics, as ordered by TC-W2V topic coherence. For each dynamic topic, we report a manually-assigned short label, the top 10 terms, coherence, and the frequency of the topic (\ie number of time windows in which it appeared).}
\end{table*}

\newpage
\begin{table*}[h]
\centering
\scriptsize{
\begin{tabular}{|l|l|l|c|c|}
\hline
\textbf{Topic} & \textbf{Short Label}     & \textbf{Top 10 Terms}                                                                       & \textbf{Freq.} & \textbf{Coh.} \\\hline
1              & Plenary administration   & president, european, political, resumption, resolution, continuation, business, adoption, union, ppe & 57             & 0.21          \\
2              & Human rights             & rights, human, fundamental, freedom, democracy, law, charter, resolution, union, violation           & 52             & 0.43          \\
4              & Gender equality          & woman, equality, gender, equal, violence, discrimination, against, work, opportunity, life           & 50             & 0.38          \\
6              & Energy                   & energy, gas, renewable, efficiency, supply, source, electricity, market, target, project             & 36             & 0.47          \\
7              & Consumer protection      & consumer, market, protection, internal, labelling, credit, regulation, single, product, network      & 36             & 0.35          \\
8              & Fisheries                & fishery, fishing, fish, stock, fisherman, fleet, sea, common, policy, measure                        & 34             & 0.43          \\
19             & Social policy            & social, employment, economic, worker, policy, labour, growth, economy, pension, jobs                 & 34             & 0.39          \\
5              & Commission questions     & commission, commissioner, work, legislative, reform, subject, programme, case, annex, censure        & 30             & 0.24          \\
12             & Budget                   & budget, draft, financial, eur, general, budgetary, section, committee, money, fund                   & 28             & 0.28          \\
22             & Agriculture              & agricultural, farmer, rural, agriculture, cap, milk, production, market, development, common         & 27             & 0.38          \\
9              & Council Presidency       & council, presidency, minister, brussels, european, regulation, common, cod, subject, summit          & 24             & 0.21          \\
10             & Liberalising services    & service, market, public, postal, competition, internal, interest, liberalisation, sector, general    & 23             & 0.38          \\
49             & Regional funds           & policy, region, cohesion, development, regional, strategy, structural, fund, economic, area          & 22             & 0.39          \\
14             & Future of Europe         & europe, union, european, states, citizen, enlargement, government, constitution, candidate, policy   & 22             & 0.26          \\
39             & Education and culture     & programme, education, culture, language, cultural, youth, sport, learning, young, training           & 21             & 0.43          \\
15             & Turkish accession        & turkey, turkish, accession, progress, cyprus, negotiation, union, membership, croatia, macedonia     & 20             & 0.41          \\
13             & Transport                & transport, railway, rail, passenger, road, network, freight, system, train, infrastructure           & 19             & 0.54          \\
32             & Trade WTO and aid    & trade, wto, world, development, developing, international, negotiation, aid, free, relation          & 19             & 0.39          \\
17             & CFSP                     & security, policy, defence, common, foreign, military, nato, immigration, aspect, european            & 19             & 0.39          \\
25             & Justice and home affairs & committee, affairs, legal, petition, regulation, internal, ombudsman, market, citizen, statute       & 19             & 0.29\\\hline         
\end{tabular}
}
\caption{List of top 20 dynamic topics, as ordered by their frequency (\ie number of time window in which a dynamic topic appears). For each dynamic topic, we report a manually-assigned short label, the top 10 terms, frequency, and TC-W2V topic coherence.}
\end{table*}


\begin{table*}[h]
\centering
\scriptsize{
\begin{tabular}{|l|l|c|}
\hline
\textbf{Taxonomy Subject}                                     & \textbf{Matched Topic Top 10 Terms}                                                                           & \textbf{Sim.} \\\hline
1.10 Fundamental Rights In The Union                 & rights, human, fundamental, freedom, democracy, law, charter, resolution, union, violation                    & 0.66          \\
4.40 Education, Vocational Training \& Youth                 & programme, education, culture, language, cultural, youth, sport, learning, young, training                    & 0.63          \\
5.20 Monetary Union                                           & euro, economic, growth, stability, pact, bank, policy, monetary, economy, ecb                                 & 0.62          \\
4.70 Regional Policy                                          & policy, region, cohesion, development, regional, strategy, structural, fund, economic, area                   & 0.62          \\
3.50 Research \& Technological Development               & research, programme, innovation, framework, funding, industry, technology, development, cell, institute       & 0.57          \\
3.60 Energy Policy                                            & energy, gas, renewable, efficiency, supply, source, electricity, market, target, project                      & 0.53          \\
6.10 Common Foreign \& Security Policy               & security, policy, defence, common, foreign, military, nato, immigration, aspect, european                     & 0.52          \\
3.20 Transport Policy in General                              & transport, railway, rail, passenger, road, network, freight, system, train, infrastructure                    & 0.51          \\
4.60 Consumers' Protection in General                         & product, medicinal, medicine, tobacco, labelling, safety, consumer, regulation, organic, advertising          & 0.50          \\
3.70 Environmental Policy                                     & waste, recycling, directive, packaging, management, environment, electronic, fuel, environmental, radioactive & 0.50          \\
8.70 Budget of the Union                                      & budget, draft, financial, eur, general, budgetary, section, committee, money, fund                            & 0.49          \\
3.15 Fisheries Policy                                         & fishery, fishing, fish, stock, fisherman, fleet, sea, common, policy, measure                                 & 0.48          \\
8.20 Enlargement of the Union                                 & romania, accession, bulgaria, enlargement, progress, croatia, union, corruption, reform, romanian             & 0.47          \\
2.50 Free Movement of Capital                                 & financial, crisis, economic, market, european, supervision, bank, perspective, fund, banking                  & 0.44          \\
2.70 Taxation                                                 & tax, vat, taxation, rate, system, fraud, states, evasion, car, transaction                                    & 0.44          \\
7.10 Free Movement \& Integration                            & border, schengen, system, states, asylum, si, area, acquis, application, immigration                          & 0.41          \\
4.50 Tourism                                                  & china, textile, chinese, industry, relation, sector, clothing, arm, import, tourism                           & 0.39          \\
3.40 Industrial Policy                                        & china, textile, chinese, industry, relation, sector, clothing, arm, import, tourism                           & 0.38          \\
4.45 Common Cultural Area                 & programme, education, culture, language, cultural, youth, sport, learning, young, training                    & 0.36          \\
3.10 Agricultural Policy \& Economies                        & animal, welfare, protection, meat, scientific, feed, ban, transport, control, plant                           & 0.36\\\hline          
\end{tabular}
}
\caption{List of top 20 legislation taxonomy subjects with corresponding matching dynamic topic, and cosine similarity of the match.}
\label{tab:match}
\end{table*}


